Measuring Sample Quality with Diffusions

Stein's method for measuring convergence to a continuous target distribution relies on an operator characterizing the target and Stein factor bounds on the solutions of an associated differential equation. While such operators and bounds are readily available for a diversity of univariate targets, few multivariate targets have been analyzed. We introduce a new class of characterizing operators based on Ito diffusions and develop explicit multivariate Stein factor bounds for any target with a fast-coupling Ito diffusion. As example applications, we develop computable and convergence-determining diffusion Stein discrepancies for log-concave, heavy-tailed, and multimodal targets and use these quality measures to select the hyperparameters of biased Markov chain Monte Carlo (MCMC) samplers, compare random and deterministic quadrature rules, and quantify bias-variance tradeoffs in approximate MCMC. Our results establish a near-linear relationship between diffusion Stein discrepancies and Wasserstein distances, improving upon past work even for strongly log-concave targets. The exposed relationship between Stein factors and Markov process coupling may be of independent interest.

==> diffusion_invariant_distribution_proof.tex <==
%

%
\section{Proof of \thmreflow{invariance}}
\label{sec:invariance-proof}

%
\begin{proof}
Suppose that conditions \eqnref{drift} and \eqnref{nonrev} hold, then  since the drift and diffusion coefficients are locally Lipschitz and the process $\process{t}{x}$ is nonexplosive, then $\process{t}{x}$ is a Markov process which solves the martingale problem \citep{EthierKu86} for the operator
\baligns
\genarg{f}{x} = \inner{\grad}{p(x) a(x) \grad f(x)}/p(x) + \half \inner{c(x)}{\grad f(x)}\qtext{for all} x\in\reals^d
\ealigns
with domain $\dom({\generator{}}) = C^2_0(\reals^d)$, since $p$ is everywhere positive.  Moreover, for all $f\in \dom(\generator{})$ we obtain
\balign
\label{eqn:invariance_test}
\Esubarg{P}{\genarg{f}{Z}}
  = \int \inner{\grad}{p(x) a(x) \grad f(x)}\,dx
  + \half \int \inner{c(x)}{\grad f(x)} p(x)\,dx.
\ealign
Since $x\mapsto p(x) a(x) \nabla f(x)$ is continuously differentiable with compact support, the first term on the right--hand side of
this equality will be zero by the divergence theorem. Similarly, the divergence theorem and the property \eqnref{nonrev}
imply that the second righthand side term is zero.  
\\\\
To prove the converse, we suppose that $P$ is an invariant distribution of the diffusion and define
\baligns
c = b - a \grad \log p  + \inner{\grad}{a} = b - \frac{\inner{\grad}{pa}}{p}.
\ealigns
Given $f \in C_0^2(\reals^d)$ , by the invariance of $P$,
\baligns
  0 &= \int \left(\inner{b(x)}{\grad f(x)} + \inner{a(x)}{\Hess f(x)}\right ) p(x)\,dx \\
  &= \int \inner{\grad f(x)}{b(x) - \frac{\inner{\grad}{a(x)p(x)}}{p(x)}} p(x)\,dx \\
  &= \int \inner{\grad f(x)}{c(x)}p(x)\, dx 
  = \int f(x) \inner{\grad}{p(x) c(x)} \, dx,
\ealigns
where we use the fact that $p$ and $a$ are continuously differentiable
and that $f$ has compact support to integrate by parts in the last equality.
Since $f\in C^2_0(\reals^d)$ is arbitrary, it follows that \eqnref{nonrev}
holds. Finally, the antisymmetric part of $\mathcal{A}$ in $L^2(p)$ is
 $f\mapsto\inner{c}{\grad f}$, so $\mathcal{A}$ is reversible
if and only if $c$ = 0.
\end{proof}


==> langevin_decay_proof.tex <==
%
%
\section{Proof of \thmreflow{langevindecay}}\label{sec:secondlangevin}

\global\long\def\yl{Y}
 \global\long\def\vl{V}
 We will establish exponential decay for the synchronous coupling of two second-order Langevin diffusions \diffref{underdamped},
 $\ensuremath{\fullprocess{z_{0}}=((\yl_{t},\vl_{t}))_{t\geq0}} \text{ and }\ensuremath{\fullprocess{z_{0}'}=((\yl_{t}',\vl_{t}'))_{t\geq0}}$,
with the same driving Wiener process $(W_t)_{t\geq0}$ and starting points $z_{0}, z_{0}'\in \reals^{2d}$.
We use the abbreviation $\nabla U=-\nabla\log p$ and solve explicitly for $\vl_{t}$ in terms of $\yl_{t}$
\balignst
\vl_{t} = \vl_{0}e^{-t}-\int_{0}^{t}e^{-(t-s)}\nabla U(\yl_{s})ds  +\sqrt{2}\int_{0}^{t}e^{-(t-s)}dW_{s}.
%
\ealignst
Following the approach of \citep[Prop 2.14]{lelievre2010free}, we obtain the expression for $\yl_{t}$,
\balignst
\yl_{t} & =\yl_{0}+\int_{0}^{t}\vl_{0}e^{-s}ds-\int_{0}^{t}\int_{0}^{s}e^{-(s-r)}\nabla U(\yl_{r})drds +\sqrt{2}\int_{0}^{t}\int_{0}^{s}e^{-(s-r)}dW_{r}ds\\
 & =\yl_{0}+\vl_{0}(1-e^{-t})-\int_{0}^{t}(1-e^{-(t-r)})\nabla U(\yl_{r})dr +\sqrt{2}\int_{0}^{t}(1-e^{-(t-r)})dW_{s}.
\ealignst
Similar expressions hold for $\yl_{t}^{\prime}$ and $\vl_{t}^{\prime}$ allowing us to compute as follows
\balignst
\yl_{t}-\yl_{t}^{\prime}  =\underbrace{\yl_{0}-\yl_{0}^{\prime}+(\vl_{0}-\vl_{0}^{\prime})(1-e^{-t})}_{\rho(t)}-\int_{0}^{t}(1-e^{-(t-r)})\left[\nabla U(\yl_{r})-\nabla U(\yl_{r}^{\prime})\right].
\ealignst
Applying the $k$-strong convexity of $U$, we find that
\balignst
%
\twonorm{\yl_{t}-\yl_{t}^{\prime}}^{2}\leq & \twonorm{\rho(t)}^{2}-2k\int_{0}^{t}(1-e^{-(t-r)})\twonorm{\yl_{r}-\yl_{r}^{\prime}}^{2}dr,
\ealignst
so that \lemsref{underdampODE} and \lemssref{underdampODEComp} yield
\balign \label{eq:posbound}
\twonorm{\yl_{t}-\yl_{t}^{\prime}}^{2}\leq 8 \twonorm{z_0-z_0^{\prime}}^{2} e^{-\frac{1}{3}t(1-\sqrt{\max\left(0,1-8k\right)})}
\ealign
where we used that $\twonorm{\rho(t)}^{2}\leq 2 \twonorm{z_0-z_0^{\prime}}^{2}$ by Jensen's inequality. Again using Jensen's inequality, we obtain the bound 
\balignst
\twonorm{\vl_{t}-\vl_{t}^{\prime}}^{2} & \leq 2\twonorm{\vl_{0}-\vl_{0}^{\prime}}^{2}e^{-2t}+2t^{2}\left\lVert{\frac{1}{t}\int_{0}^{t}e^{-(t-s)}\nabla U(\yl_{s})-\nabla U(\yl_{s}^{\prime})}\ds\right\rVert_{2}^{2}\\
 & \leq2\twonorm{\vl_{0}-\vl_{0}^{\prime}}^{2}e^{-2t}+2t\int_{0}^{t}e^{-2(t-s)}M_2(\log p)\twonorm{\yl_{s}-\yl_{s}^{\prime}}^{2}\,ds
\ealignst
where we used that $\nabla U$ has Lipschitz constant $M_2(\log p)$. 
Combining \eqref{eq:posbound} with this inequality and letting $\lambda_{1}=\frac{1}{3}(1-\sqrt{\max\left(0,1-8k\right)})$, we obtain
%
\begin{align*}
\twonorm{\vl_{t}-\vl_{t}^{\prime}}^{2}  &\leq2\twonorm{\vl_{0}-\vl_{0}^{\prime}}^{2}e^{-2t}+16M_2(\log p)t\frac{1}{2+\lambda_{1}}e^{-\lambda_{1}t}\twonorm{z_{0}-z_{0}^{\prime}}^{2}\\
 &\leq (8M_2(\log p)+2)te^{-\lambda_{1}t}\twonorm{z_{0}-z_{0}^{\prime}}^{2}
\end{align*}
The theorem is proved by combining this bound with equation (\ref{eq:posbound}).
%
%
%
%
%
%

%
\begin{lemma} \label{lem:underdampODE}
The integral equation
$%
u(t)=u(0)-2k\int_{0}^{t}(1-e^{-(t-r)})u(r)\,dr
$
has a solution satisfying
\balignst
u(t)  =u(0)e^{-\frac{t}{2}}(\cosh\left(\frac{t}{2}\sqrt{1-8k}\right)+\frac{\sinh\left(\frac{t}{2}\sqrt{1-8k}\right)}{\sqrt{1-8k}})\label{eq:underdampedUpper}
  \leq 4 u(0)e^{-\frac{1}{3}t(1-\sqrt{\max\left(0,1-8k\right)})}.
\ealignst
\end{lemma}
%
%
\begin{proof} Taking a derivative with respect to
$t$, we obtain
\balignst
u'(t) & =-2k u(t)-{2k}\int_{0}^{t}e^{-(t-r)}u(r)\,dr+2k e^{-(t-t)}u(t)\\
 & =-{2k}\int_{0}^{t}e^{-(t-r)}u(r)\,dr
 =-{2k}(H\star u)(t),\quad t>0,
\ealignst
where $H(t)=e^{-t}$. Taking the Laplace transform on both sides, we obtain
\baligns
s\hat{u}(s)-u(0)=-2k\hat{H}(s)\hat{u}(s),\text{with }\hat{H}(s)=\left(s+1\right)^{-1}.
\ealigns
It follows that for $s>0$, $\textstyle\hat{u}(s)=\frac{u(0)}{s+2k\left(s+1\right)^{-1}}.$
Taking the inverse Laplace transform yields the expression for $u$. %
\global\long\def\sing{\tau}

To compute the bound, let $\sing=\frac{9}{8}$. In the following we use the fact that if $\log p$
is $k$-strongly concave, then it is also $\tilde{k}$-strongly
concave for $\tilde{k}<k$. 
We also use that $\sinh x\leq e^{x}$
and $\cosh x\leq e^{x}$ for $x\ge0$. 
For $k\leq\frac{1}{8\sing}$, we have 
\baligns
u(t) & \leq u(0)(1+\left(1-{\sing}^{-1}\right)^{-\frac{1}{2}})e^{-\frac{t}{2}(1-\sqrt{1-8k})}
  \leq4u(0)e^{-\frac{t}{3}(1-\sqrt{\max\left(0,1-8k\right)})}.
\ealigns
For $k>\frac{\sing}{8}$, we notice $\cosh ix=\cos x$ and $\sin ix=i\sin x$, so
\[
u(t)\leq u(0)(1+\sqrt{\sing-1})e^{-\frac{t}{2}}\leq4u(0)e^{-\frac{t}{3}(1-\sqrt{\max\left(0,1-8k\right)})}.
\]
For $\frac{1}{8\sing}<k\leq\frac{\sing}{8}$, we can use the case $k\leq\frac{1}{8\sing}$  because $\log p$ is $\frac{1}{8\sing}$-strongly concave. The result now follows since
\balignst
\frac{t}{2}(1-\sqrt{1-8k})\ge\frac{t}{2}(1-\sqrt{1-\frac{1}{\tau}})\ge\frac{t}{3}\ge\frac{t}{3}(1-\sqrt{\max\left(0,1-8k\right)}).
\ealignst

%
%
%
%
%
%
%
%
%
%
\end{proof}
%

\begin{lemma} \label{lem:underdampODEComp} If
$
z(t)\leq c-2k\int_{0}^{t}(1-e^{\left(-(t-r)\right)})z(r)dr,
$ then $z(t)\leq u(t)$ for $u(t)$ defined by 
\balignt
\label{eqn:ode_gronwall}
u^{\prime}(t)  = 2k\int_{0}^{t}\left(1-e^{-(t-r)}\right)u(r)dr\text{ and }u(0)=c.
\ealignt

\end{lemma} \begin{proof} Let $\Phi(u,t)=2k\int_{0}^{t}\left(1-e^{-(t-r)}\right)u(r)dr$.
Let $u_{n}$ be the solution to 
\begin{equation*}\textstyle
u_{n}^{\prime}(t)=\Phi(u_{n},t)+\frac{1}{n}.%
\end{equation*}
If $z\leq u_{n}$ we are done. Otherwise there is $t_{1}\in(0,T)$
such $z(t_{1})>u_{n}(t_{1})$ and, since $z$ and $u_n$ are continuous,
a largest $t_{2}\in[0,t_{1})$
such that $z(s)\leq u_{n}(s)$ for $s\leq t_{2}.$ 
By continuity, there is a $\delta$ such that $z(s)>u(s)$
for $s\in[t_{2},t_{2}+\delta)$, 
\baligns\textstyle
\frac{z(t_{2}+h)-z(t_{2})}{h}>\frac{u(t_{2}+h)-u(t_{2})}{h}.
\ealigns
Hence $\frac{d}{dt}z(t_{2})>\Phi(u_{n},t_{2})+\frac{1}{n}\ge\Phi(z,t_{2})+\frac{1}{n}$.
Thus, there is a contradiction because of the monotonicity of $\Phi$.  It follows that $z \leq u_n$ for all $n > 0$.  Taking $n\rightarrow\infty$ the solution $u_{n}$ converges to a solution $u^{\star}$ of \eqnref{ode_gronwall}, see proof of Lemma 2.7 in \cite{robinson2001Infinite}. Since equation \eqref{eqn:ode_gronwall} has a unique solution, obtained by taking Laplace transforms as in Lemma \ref{lem:underdampODE} it follows that $z(t) \leq u(t)$.
\end{proof}


==> nonuniform_stein_sets_proof.tex <==
%

\section{Proof of \propreflow{stein-equiv}} \label{sec:stein-equiv-proof}

Fix any $c_1, c_2, c_3 > 0$ and let $c_{min} = \min(c_1, c_2, c_3)$ and
$c_{max} = \max(c_1, c_2, c_3)$. Then by the linearity of differentiation,
we have that $c_{min}\steinset \subseteq \steinset^{c_{1:3}}$ and similarly
$\steinset^{c_{1:3}} \subseteq c_{max}\steinset$. Since the Stein
discrepancy's objective is linear in $g$ for a fixed target distribution
$P$, the first relation implies that
\baligns
\diffstein{Q_n}{\steinset^{c_{1:3}}} \ge \diffstein{Q_n}{c_{min}\steinset} =
c_{min} \diffstein{Q_n}{\steinset}.
\ealigns
Using a similar argument, the latter relation implies
$\diffstein{Q_n}{\steinset^{c_{1:3}}} \leq c_{max}\diffstein{Q_n}{\steinset}$,
concluding the proposition.


==> spanner_stein_equivalence_proof.tex <==
%
%
\section{Proof of \propreflow{spanner-equivalence}} \label{sec:spanner-equivalence-proof}
Since the diffusion Stein discrepancy objective is linear in $g$ and depends on $g$
only through the values $g(x_i)$ and $\grad g(x_i)$, the proofs of \citep[Prop. 5 and 6]{GorhamMa15} directly imply the result.

%
\lester{Let's move this section to a separate file}
\section{Contraction of the Second-Order Langevin Equation }\label{app:underdamped}
\lester{Does anyone know how to fix the weird centering behavior of long appendix titles?}
We consider Equation \eqref{eq:sde-underdamped}  with $\Gamma=I$ which gives rise to 
\begin{align*}
dq_{t} & =v_{t}dt\\
\epsilon dv_{t} & =-\nabla V(q_{t})dt-v_{t}dt+\sqrt{2}dW_{t}
\end{align*}
Notice that we can solve for $v_{t}$ explicitly 
\begin{align}
\label{eq:underdampedVelocity}
\begin{aligned}
v_{t}=&v_{0}\exp{\left(-\frac{t}{\epsilon}\right)}-\epsilon^{-1}\int_{0}^{t}\exp{\left(-(t-s)/\epsilon\right)}\nabla V(q_{s})ds
&+\epsilon^{-1}\sqrt{2}\int_{0}^{t}\exp{\left(-(t-s)/\epsilon\right)}dW_{s}.
\end{aligned}
\end{align}
This allows us to obtain an expression for $q_t$
\begin{align*}
q_{t} & =q_{0}+\int_{0}^{t}v_{0}\exp{\left(-s/\epsilon\right)}ds-\epsilon^{-1}\int_{0}^{t}\int_{0}^{s}\exp{\left(-(s-r)/\epsilon\right)}\nabla V(q_{r}^{\epsilon})drds\\
 & +\epsilon^{-1}\sqrt{2}\int_{0}^{t}\int_{0}^{s}\exp{\left(-(s-r)/\epsilon\right)}dW_{r}ds\\
 & =q_{0}+v_{0}\epsilon(1-\exp{\left(-t/\epsilon\right)})-\int_{0}^{t}(1-\exp{\left(-(t-r)/\epsilon\right)})\nabla V(q_{r}^{\epsilon})dr\\
 & +\sqrt{2}\int_{0}^{t}(1-\exp{\left(-(t-r)/\epsilon\right)})dW_{s}
\end{align*}

Let $q_{t}$ and $q_{t}^{\prime}$ correspond to the initial conditions $(q_{0},p_0)$ and 
and $(q_{0}^{\prime},p_{0}^{\prime})$, respectively. We compute an expression for $\left|q_{t}-q_{t}^{\prime}\right|^{2}$ as follows

\begin{align*}
q_{t}-q_{t}^{\prime} & =A-\int_{0}^{t}(1-\exp{\left(-(t-r)/\epsilon\right)})\left[\nabla V(q_{r}^{\epsilon})-\nabla V(q_{r}^{\prime\epsilon})\right]\\
\left|q_{t}-q_{t}^{\prime}\right|^{2}= & \left\Vert A\right\Vert^{2}-2\int_{0}^{t}(1-\exp{\left(-\left(t-r\right)/\epsilon\right)}\left[\nabla V(q_{r}^{\epsilon})-\nabla V(q_{r}^{\prime\epsilon})\right]\cdot\left[q_{r}^{\epsilon}-q_{r}^{\prime\epsilon}\right]dr \\
\left|q_{t}-q_{t}^{\prime}\right|^{2} & \leq\left[\underbrace{(q_{0}-q_{0}^{\prime})+(v-v_{0}^{\prime})\epsilon(1-\exp{-t/\epsilon})}_{\rho(t)}\right]^{2}\\
 & -2\kappa\int_{0}^{t}(1-\exp{-(t-r)\epsilon})\left|q_{r}-q_{r}^{\prime}\right|^{2}dr.
\end{align*}
where we use the strong convexity of $V$.
Combining the two lemmas below we achieve that

\[
\left|q_{t}-q_{t}^{\prime}\right|^{2}\leq\twonorm{q_{t}-q_{t}^{\prime}}^{2}(1+\epsilon)+(\epsilon+\epsilon^{2})\twonorm{v_{0}-v_{0}^{\prime}}^{2})U(\kappa,\epsilon,t).
\]

This can be used to obtain a bound on
\begin{align*}
\E \twonorm{|v_{t}-v_{t}^{\prime}}^{2} & \leq2\left|v_{0}-v_{0}^{\prime}\right|^{2}\exp{\left(-2\frac{t}{\epsilon}\right)}+2\epsilon^{-2}t^{2}\left|\int_{0}^{t}\exp{\left(-(t-s)/\epsilon\right)}\left(\nabla V(q_{s})-\nabla V(q_{s}^{\prime})\right)\frac{ds}{t}\right|^{2}\\
& \leq2\left|v_{0}-v_{0}^{\prime}\right|^{2}\exp{\left(-2\frac{t}{\epsilon}\right)}+2\epsilon^{-2}t^{2}\int_{0}^{t}\exp{\left(-2(t-s)/\epsilon\right)}L\left|q_{s}-q_{s}^{\prime}\right|^2\frac{ds}{t}
\end{align*}



\begin{lemma} \label{lem:underdampODE}Consider the integral equation
\[
u(t)=u(0)-2\kappa\int_{0}^{t}(1-e^{-(t-r)/\epsilon})u(r)\,dr.
\]
Then the solution $u(t)$ exists and satisfies 
\begin{align}
\label{eq:underdampedUpper}
\begin{aligned}
u(t) & =\text{u(0)}\underbrace{e^{-\frac{1}{2}(t\epsilon)}\left(\cosh\left(\frac{t\sqrt{\epsilon^{4}-8\kappa\epsilon}}{2\epsilon}\right)+\frac{\epsilon^{2}\sinh\left(\frac{t\sqrt{\epsilon^{4}-8\kappa\epsilon}}{2\epsilon}\right)}{\sqrt{\epsilon^{4}-8\kappa\epsilon}}\right)}_{U(\kappa,\epsilon,t)}.\\
& =\frac{\text{u}_{0}e^{-\frac{t\left(\sqrt{\epsilon^{4}-8\kappa\epsilon}+\epsilon^{2}\right)}{2\epsilon}}\left(\sqrt{\epsilon^{4}-8\kappa\epsilon}\left(e^{\frac{t\sqrt{\epsilon^{4}-8\kappa\epsilon}}{\epsilon}}+1\right)+\epsilon^{2}\left(e^{\frac{t\sqrt{\epsilon^{4}-8\kappa\epsilon}}{\epsilon}}-1\right)\right)}{2\sqrt{\epsilon^{4}-8\kappa\epsilon}}
\end{aligned}
\end{align}

\end{lemma} 
\begin{proof}
Taking the derivative with respect to $t$ we obtain: 
\begin{align}
u'(t) & =-2\kappa u(t)-\frac{2\kappa}{\epsilon}\int_{0}^{t}e^{-(t-r)/\epsilon}u(r)\,dr+2\kappa e^{-(t-t)/\epsilon}u(t)\\
& =-\frac{2\kappa}{\epsilon}\int_{0}^{t}e^{-(t-r)/\epsilon}u(r)\,dr\\
& =-\frac{2\kappa}{\epsilon}H*u(t),\quad t>0,
\end{align}

where $H(t)=\exp(-t/\epsilon)$. Taking Laplace transform on both
sides we obtain: 
\[
s\hat{u}(s)-u(0)=-\frac{2\kappa}{\epsilon}\hat{H}(s)\hat{u}(s),
\]
where 
\[
\hat{H}(s)=\left(s+\epsilon^{-1}\right)^{-1}.
\]
It follows that, for $s>0$: 
\[
\hat{u}(s)=\frac{u(0)}{s+\frac{2\kappa}{\epsilon}\left(s+\epsilon^{-1}\right)^{-1}}.
\]
Taking the inverse Laplace transform completes the proof.
\end{proof}

\begin{lemma}
\label{lem:underdampODEComp}Suppose that 
\[
z(t)\leq c+-2\kappa\int_{0}^{t}(1-\exp{\left(-(t-r)\epsilon\right)})z(r)dr
\]
then $z(t)\leq u(t)$ which satisfies 
\begin{align*}
u^{\prime}(t) & =\int_{0}^{t}\left(1-e^{-(t-r)/\epsilon}\right)u(r)dr
\end{align*}
with $u(0)=c$ 
\end{lemma}
\begin{proof}
Define $\Phi(u,t)=\int_{0}^{t}\left(1-e^{-(t-r)/\epsilon}\right)u(r)dr$.
Let $u_{n}$ be the solution to 
\[
u_{n}^{\prime}(t)=\Phi(u_{n},t)+\frac{1}{n}
\]
If $z\leq u_{n}$ we are done. Otherwise there is $t_{1}\in(0,T)$
such $z(t_{1})>y_{n}(t_{1})$. Thus there is $t_{2}\in[0,t_{1}$ largest
such that $z(s)\leq u_{n}(s)$ for $s\leq t_{2}.$ Since $z$ and
$u_{n}$ are continuous there is a $\delta$ such that $z(s)>u(s)$
for $s\in[t_{2},t_{2}+\delta$ 
\[
\frac{z(t_{2}+h)-z(t_{2})}{h}>\frac{u(t_{2}+h)-u(t_{2})}{h}.
\]
Hence $\frac{d}{dt}z(t_{2})>\Phi(u_{n},t_{2})+\frac{1}{n}\ge\Phi(z,t_{2})+\frac{1}{n}$.
Thus, there is  a contradiction because of the monotonicity of $\Phi.$ 
\andrew{One more step needed in the argument.  One must appeal to compactness, e.g. Arzela Ascoli.}
\end{proof} 
%

